JWST/NIRSpec Detects Warm CO Emission in the Terrestrial-Planet Zone of HD 131488

We have obtained a high-resolution, JWST NIRSpec $2.87$ -- $5.14$ $\mu$m spectrum of the debris disk around HD 131488. We discover CO fundamental emission indicating the presence of warm fluorescent gas within $\sim10$ AU of the star. The large discrepancy in CO's vibrational and rotational temperature indicates that CO is out of thermal equilibrium and is excited with UV fluorescence. Our UV fluorescence model gives a best fit of $1150\,$K with an effective temperature of $450$, $332$, and $125\,$K for the warm CO gas kinetic temperature within $0.5$, $1$, and $10\,$AU to the star and a gas vibrational temperature of $8800\,$K. The newly discovered warm CO gas population likely resides between sub-AU scales and $\sim\,10\,$AU, interior to the cold CO reservoir detected beyond $35\,$AU with HST STIS and ALMA. The discovery of warm, fluorescent gas in a debris disk is the first such detection ever made. The detection of warm CO raises the possibility of unseen molecules (H$_2$O, H$_2$, etc) as collisional partners to excite the warm gas. We estimated a lower mass limit for CO of $1.25\times 10^{-7}\text{M}_{\oplus}$, which is $10^{-5}$ of the cold CO mass detected with ALMA and HST. We demonstrate that UV fluorescence emerges as a promising avenue for detecting tenuous gas at $10^{-7}$ Earth-mass level in debris disks with JWST.

==> deleted.tex <==


Signatures of UV fluorescence of warm gas can also be observed from individual spectral lines that are both highly vibrationally excited and rotationally excited. As shown earlier in Figure \ref{fig:examples} ROI~3, we see many lines in the $4.8\,$--$5.1\,\mu$m region that are of high v and high J. ROI~3 shows examples of v(7-6) J(17-16), v(4-3) J(6-5), v(6-5) J(7-6) of $^{12}$CO ro-vibrational emission. Similarly, the lines in blue shades in ROI~3 are, $^{13}$CO ro-vibrational emission lines with high J and high v, but not annotated to avoid clutter. We provide the data behind Figure \ref{fig:vib-Levels} for interested readers. Through these high J high v line detections, we confirm the existence of UV fluorescence of warm CO gas in HD 131488. 


\added{Comparing our estimated dust mass and dust locations with ground-based coronagraphic studies on the system, we find that we are probing dust in the region occulted by the coronagraph, regardless of the assumptions on dust properties.} We calculate the equivalent distance of \added{a} $273\,$K grain in thermal equilibrium to approximate the location of the water-ice line. The corresponding distances for large and small grains are $5.3$ and $30.2\,$AU. Comparing the locations of the grains with a temperature where water-ice freezes out, we infer that the warm grains entrained in the newly discovered warm gas most likely reside inside the water-ice line in this planetary system, which is inaccessible to ground-based coronagraphic images. We compare our estimated dust distance to the peak locations (at $10$ and $100$ AU) of the warm and cold belts shown in Fig. 15 of \citet{Pawellek+24}. We find that in either case -- assuming blackbody or the small grain limit, the observed warm and gas dust is most likely located within the warm belt. In addition, SED analyses in past studies of the system \citep{Melis+13, Lisse+17} have revealed a hot dust excess at $3$--$4\,\mu$m, pointing to the existence of hot and cool dust in the inner disk at $\sim\,6\,$AU and $\sim35\,$AU. The warm CO gas could be co-located with the $6\,$AU dust population.

\item \textcolor{red}{Check inconsistencies: Tvib is not fitted} We require the vibrational temperature ($T_{vib}$) of the warm/hot CO population to range from $80$ to $9000$\,K. The upper bound reflects the diluted color-temperature ($\sim9000$\,K) of the radiation field around the star. The lower bounds of $T_{vib}$ and $T_{rot}$ are chosen to be above the upper bounds of $T_{abs}$, a physical condition required for gas emission.

The last factor we considered is the \added{the effective radius for the cold CO foreground absorption. At the initial stage of modeling, we simply assume that the cold gas seen in absorption is perfectly co-located with warm gas seen in emission. However, this naive assumption resulted in the overprediction of the absorption line depth. Previous works have found that even a small misalignment (as small as 2 degrees) between disk position angle from a perfectly edge-on angle could result in non-detection of absorption for debris disks with ALMA CO emission detection \citep[e.g.,][]{Worthen+24}. Inspired by this past work, we try to refine our model by adding a description of the effective CO absorption radius, and the addition of which largely improves the absorption modeling. As illustrated in Fig. \ref{fig:cartoon}, the} foreground gas component no longer aligns with the warm \added{gas} geometrically at a certain radial distance along the line of sight. We use $R_{\textrm{absorption}}$ to describe the effective radius of such a radial distance. \added{We model $R_{\textrm{absorption}}$ by fitting for $N_{\textrm{absorption}}$, which follows the same convention as $N_{\textrm{rings}}$. $N_{\textrm{absorption}}$ is taken to be $0.1\,$AU within $1$\,AU and $1\,$AU wide for radius beyond $1\,$AU. }


% We consider the geometry of the emitting area as a third factor. As shown in Fig 
% \ref{fig:cartoon}, a cartoon of our model, we fitted for the inner edge ($a_0$),  and the number of rings ($N$), assuming the ring width (dr) is $0.1\,$AU wide from $0.1$ to $1\,$AU and increases to $1\,$AU wide outward of $1\, $AU. The ring width is $0.1$AU because this increment captures the radial gradient change in the gas vibrational temperature given the star's UV radiation. \added{In the} $1$ to $100\,$AU region, the gas vibrational temperature changes slowly with the radial distance, so $1\,$AU is sufficient to describe the change in the temperature changes as a function of radial distance. 

% As shown in Fig \ref{fig:cartoon}, a cartoon of our model, we fitted for the inner edge ($a_0$), and the number of rings ($N$), assuming the ring width (dr) is $0.1\,$AU wide from $0.1$ to $1\,$AU and increases to $1\,$AU wide outward of $1\, $AU. The ring width is $0.1$AU because this increment captures the radial gradient change in the gas vibrational temperature given the star's UV radiation. \added{In the} $1$ to $100\,$AU region, the gas vibrational temperature changes slowly with the radial distance, so $1\,$AU is sufficient to describe the change in the temperature changes as a function of radial distance. 


Firstly, we demonstrate that multiple vibrational levels of $^{12}$CO and $^{13}$CO are observed, which implies the UV fluorescence mechanism at play. In Figure \ref{fig:vib-Levels} middle and bottom panels, we show a total of $10$ vibrational levels from v(1-0) to v(10-9) for $^{12}$CO emission, and $5$ levels of $^{13}$CO emission from vibrational excitation are observed. Each level is annotated and offset to avoid overcrowding the plot. The relative strengths for emission lines of each vibrational level are true to scale but offset for clarity. To avoid clutter, we show all the vibrational levels for $^{12}$CO here in solid curves, and all vibrational levels for $^{13}$CO in blue shades. In Figure \ref{fig:examples} top panel, we annotate a few regions of interest (ROI). ROI 1 is an example to demonstrate the effect of blended lines. For each emission line in the observed spectrum, its central wavelength corresponds to the central wavelengths for multiple lines at various vibrational and rotational levels. The Figure \ref{fig:examples} middle panel shows that for the leftmost emission line, we see three lines contributing to the overall observed flux. These lines include the ground state vibrational v(1-0) emission with J(1-0), the 2nd excited vibrational state v(2-1) with J(5-4) and the third excited vibrational state v(3-2) with high J lines, J(13-12). Similarly, for the observed lines with a central wavelength of $4.6911\mu$m, multiple levels of vibrationally excited lines have a central wavelength close to $4.6911\mu$m. We describe the line blending issue quantitatively in subsection \ref{sec:line-flux}. 


% Secondly, we show the presence of $^{13}$CO alongside $^{12}$CO species, because $^{12}$CO alone cannot explain the line ratios observed in the spectra. ROI 2 in Figure \ref{fig:examples} (bottom left) demonstrates the relative contributions of $^{12}$CO and $^{13}$CO. For visualization purposes, all $^{13}$CO emission lines are shaded in blue regardless of their vibrational energy level, and the colors for $^{12}$CO lines follow the color palette for vibrational energy levels in Figure \ref{fig:vib-Levels}. With all the lines weighted by their SNR, we fit for a $^{12}$CO/$^{13}$CO istopologue ratio. We discuss our approaches in detail in section \ref{sub:CO-model} and the implications in section \ref{sub:gasimplications}.
 
% Additionally, we show that CO gas is emitting at both warm and cold temperatures by identifying some highly excited rotational emission lines in addition to the ground state transitions as demonstrated in ROI~1. In Figure \ref{fig:examples} bottom right panel, we annotate high J lines, such as v(7-6) J(17-16), v(4-3) J(5-4), v(6-5) J(7-6). The high J lines clearly show the existence of warm gas. To reconcile the warm and cold CO gas, we explore a temperature gradient and its possible geometry in section \ref{sub:geometry} and present spectra from various regions of the disk in Figure \ref{fig:COmodel}.

% Lastly, we observe hints of CO gas in absorption from the asymmetric band heads at first glance. A naive model of simply summing the flux from the middle panel of Figure \ref{fig:vib-Levels} will result in over-predicted line flux in the $4.56$\,--\,$4.7\,\mu$m  region. We leverage knowledge from STIS cold CO absorption detection of this source from \citet{Brennan+24} and explore the possible inclusion of a component of cold CO gas in the foreground to obscure and absorb the flux in the R branch locations of $^{12}$CO fundamental emission. For the cold CO absorption component, we consider the temperature and column density constrained from STIS UV observations and associated past ALMA observations in section \ref{sub:CO-model} and include a cartoon, Figure \ref{fig:cartoon}, for visualization purposes.
